An Uncertainty-Aware Approach to Optimal Configuration of Stream Processing Systems

Finding optimal configurations for Stream Processing Systems (SPS) is a challenging problem due to the large number of parameters that can influence their performance and the lack of analytical models to anticipate the effect of a change. To tackle this issue, we consider tuning methods where an experimenter is given a limited budget of experiments and needs to carefully allocate this budget to find optimal configurations. We propose in this setting Bayesian Optimization for Configuration Optimization (BO4CO), an auto-tuning algorithm that leverages Gaussian Processes (GPs) to iteratively capture posterior distributions of the configuration spaces and sequentially drive the experimentation. Validation based on Apache Storm demonstrates that our approach locates optimal configurations within a limited experimental budget, with an improvement of SPS performance typically of at least an order of magnitude compared to existing configuration algorithms.

==> sections/problem.tex <==
\section{A Case for Bayesian Optimization}
\label{sec:uncertain-measurement}


\subsection{Problem statement}

Let us consider the set of \emph{configuration parameters} as $\mathbb{D} = \{\mathbf{d}_1, \dots , \mathbf{d}_d\}$ with corresponding options (parameter values), $Dom(\mathbf{d}_i)$, with which we can tune the configuration $\mathbf{d}_i$. Therefore, we can represent the \emph{full configuration space} as $\mathbb{X}=Dom(\mathbb{D}) = Dom(\mathbf{d}_1) \times \dots \times Dom(\mathbf{d}_d)$. A \emph{subspace} of the configuration space is $Dom(\mathbf{d}_1) \times \dots \times Dom(\mathbf{d}_n)$, where each $Dom(\mathbf{d}_i)$ is a subset possible options for the corresponding parameter $Dom(\mathbf{d}_i)$. The \emph{neighborhood} of a configuration is a subspace with the configuration at its center. These mathematical structures, i.e., full configuration space, subspaces, and neighborhoods of a configuration, form hypercubes in the Hilbert space. 

We represent the performance of a \gls{sps} topology with a configuration $\mathbf{x}\in \mathbb{X}$ by $f(\mathbf{x})$. The function $f$ establish a \emph{response surface} over the full configuration space $\mathbb{X}$ by interpolation and the concept of neighborhood defined above. The response function $f$ is in principle \emph{unknown}, and the problem of finding optimal configuration boils down to find a configuration that minimizes $f$:

\begin{equation} \label{eq:reponse-function}
\mathbf{x}^*=\arg \min _{\mathbf{x}\in\mathbb{X}} f(\mathbf{x})
\end{equation}
We assume that the parameter space $\mathbb{X}$ is a bounded set $\mathbb{X}\subset{\mathbb{R}^d}$ and the function $f(\mathbf{x})$ is continuous and smooth on $\mathbb{X}$ considering that we can interpolate the response values over space $\mathbb{X}$. We also assume the response function $f$ is latency, however, without loosing the generality, we can assume $f:=-f$ in Eq. \ref{eq:reponse-function} if the response is latency.

In practice, the performance function $f(\mathbf{x})$ is often unknown or does not have a closed-form \cite{Lizotte2012}. We therefore have to model the above problem as a \emph{black-box optimization problem} where the objective function is a black-box with limited function evaluation. The challenge is to obtain the global optimal solution, since the objective function is usually multi-dimensional, highly non-linear, non-convex and multi-modal.
%Therefore, what is required is an \emph{efficient search algorithm} that obtains a good solution with a minimum number of experiments.

%To determine the response surface $f$ value at a configuration setting $\mathbf{x}$, (i) we set the topology's configuration parameters to their corresponding values in $\mathbf{x}$, (ii) deploy the topology (cf. Figure \ref{fig:system-model}) and (iii) run the topology with a specified workload for a specific period of time we set, and (iv) measure the resulting end to end latency and throughput. We refer to each such topology trial run as an experiment, and the result is a pair of $(\mathbf{x},f(\mathbf{x}))$ sample. Given the variability in stream processing systems, if we repeat each trial run several times, each time we may get a different value but within a specific confidence interval, so in this work we assume the measurements are not noise-free and contain a noise with normal distribution with zero mean and an specific variance. This assumption is the most notable differentiating factor of our approach with respect to existing work, because due to our best knowledge, there is no such configuration testing approach that explicitly assume such uncertainty in their search algorithm. Therefore, we claim for a \emph{uncertainty-aware} approach in this work.

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=5cm]{figures/boxplot-longrun-multitenant-logscale-all-captions}
		\caption{Noisy experimental measurements. Note that $+$ here means that {\sf wc} is deployed in a multi-tenant enviornment with other neighbor ropologies and due to this not only the latency is increased but also the variability of the observations is also increased.}
		\label{fig:boxplot-longrun}
	\end{center}
\end{figure}

\subsection{Trading accuracy for speed}
For configuration optimization, no matter what solution we would adopt, there is a need for some experimental measurement to provide ground truth data in order to either measure or predict the performance. In the previous section we have identified the configuration space as a major obstacle to the measurement process, together with the presence of non-linear interactions between the parameters. In order to address this issue, we propose an experimental approach that accelerates system evaluation by reducing the length of experiments, thus allowing to explore a wider range of configurations within a given time period. However, a challenge of this proposal is the increased variance observed in the recorded performance measures due to the limited sample sizes and the inherent variabilities in the workloads and the deployment environment. To illustrate measurement variabilities, we took different samples of the latency in {\sf WordCount} over 2 hours for each of the five setting. After cutting the initial 3 minutes, we then make an average over the periods afterwards, resulted in slightly over 6000 data points. In other words, we have the data associated to 6000 different testing time for the topology under test. Note that the configuration across all 5 setting are similar just the number of neighbors is different. The result in Figure~\ref{fig:boxplot-longrun} shows the minimum, maximum, median, mean and the outliers of our measurements as a function of the measurement topology, cf. Table \ref{tab:configuration-parameters}. Summarizing, we believe that experimental speedups are possible if we can deal large variabilities in the measurements, however configuration optimization procedures that cope with such variabilities are still lacking, calling for a novel approach.


\begin{table}
	\caption{Signal to noise ratios for configuration testing.}
	\resizebox{\columnwidth}{!}{%
		\begin{threeparttable}
			\begin{tabular}{lccccc}
				\toprule
				Topology & $\mu_{latency}$ & $\sigma_{noise}$ & $\mu_{ci}$ & $\sigma_{ci}$ & $\frac{\mu_{latency}}{\sigma_{noise}}$ \\
				\midrule
				{\sf wc}  & 6.07 & 0.48 & $[6.05,6.08]$ & $[0.47,0.49]$ & 12.72\\
				{\sf wc+rs}  & 9.03 & 0.99 & $[9.01,9.06]$ & $[0.97,1.00]$ & 9.16\\
				{\sf wc+sol} & 15.17 & 1.43 & $[15.14,15.21]$ & $[1.41,1.46]$ & 10.58\\
				{\sf wc+wc}  & 10.48 & 0.55 & $[10.47,10.50]$ & $[0.55,0.56]$ &18.91\\
				{\sf wc+rs+sol+wc}  & 92.00 & 88.26 & $[89.88,94.12]$ & $[86.78,89.78]$ & 1.04\\
				\bottomrule
			\end{tabular}
			\begin{tablenotes}
				\small
				\item In the last column we calculated the signal-to-noise ratio which is defined as the ratio of the power of a signal (mean of topology latency) and the power of measurement noise (unwanted signal). 
			\end{tablenotes}
		\end{threeparttable}}
		
		\label{tab:signal-to-noise}
	\end{table}



\subsection{Bayesian optimization}
%In a high-level view, existing model-based works on configuration optimization for software systems exploit the concept of regression to derive a mean of estimation for the configurations that have not been tested \cite{yigitbasi2013towards}. Other methods derive a local gradient based on few observations to search for a better configuration in the neighborhood of the already experimented ones \cite{xi2004smart}. The main commonality among these approaches is that they all based on the notion of mean estimate and this has two consequences. First, if they underestimate and use a less complex model for describing the observations, then the estimation error is high no matter how many observations made. On the other hand, if they select an over-complicated model, this leads to an overfit. Therefore, in order to estimate the optimal configuration, one needs to perform near full-factorial design in order to derive a good estimate and not to trap in a local optimum.

In this work, we exploit GP models which use both mean and variance of the estimates for configuration selections in a sequential setting. The variance of estimates play a critical role in this framework in order to not only exploit existing observations but more importantly explore zones that are likely to lead to the global optimum. %We will provide the details of Bayesian observation in Section \ref{sec:method}, however in order to better motivates this approach for configuration optimization, we figuratively demonstrates how such variance for estimates can help for excluding un-interesting zones.

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=6cm]{figures/gp-example}
		\caption{An example of 1-dimensional $\mathcal{GP}$ seven observations. The solid green line is the $\mathcal{GP}$ mean prediction of the black box function given the data, and the shaded grey area shows the confidence interval.}
		\label{fig:example-gp}
	\end{center}
\end{figure}

Figure \ref{fig:example-gp} shows a 1-dimensional response surface and its estimates. At point $x_1$ the confidence interval due to lack of observations in the neighborhood is high while the lower confidence interval in the right hand side of $x_4$ is lower and our approach correctly prioritize that zone in order to find optimum point. The confidence interval in the neighborhood of $x_2$ and $x_3$ is not high and correctly our approach does not select to explore these zones. Note that the selection of zones to test is based on some well defined criteria that will be defined in the next section.

%This figure demonstrates that with the current estimates, we do not need to investigate the area between $[0,0.9]$ any more because we know that based on the confidence interval of the estimates the minimum is not located in this interval. This is the power of confidence interval for the estimates that enable Bayesian optimization framework to skip uninteresting zones and explore the appropriate part of response surface in order to perform less experiment while get more information out of the unknown surface.

%In BO4CO, as opposed to DoE, which tries to learn the whole response surface, for configuration optimization problem, we do not need to learn the whole response function but only regions of interests (RoI). We also experimentally demonstrate that BO4CO locates all the optimum configurations when there exists multiple global optimum.


